How Gamification Affects Physical Activity: Large-scale Analysis of Walking Challenges in a Mobile Application

Gamification represents an effective way to incentivize user behavior across a number of computing applications. However, despite the fact that physical activity is essential for a healthy lifestyle, surprisingly little is known about how gamification and in particular competitions shape human physical activity. Here we study how competitions affect physical activity. We focus on walking challenges in a mobile activity tracking application where multiple users compete over who takes the most steps over a predefined number of days. We synthesize our findings in a series of game and app design implications. In particular, we analyze nearly 2,500 physical activity competitions over a period of one year capturing more than 800,000 person days of activity tracking. We observe that during walking competitions, the average user increases physical activity by 23%. Furthermore, there are large increases in activity for both men and women across all ages, and weight status, and even for users that were previously fairly inactive. We also find that the composition of participants greatly affects the dynamics of the game. In particular, if highly unequal participants get matched to each other, then competition suffers and the overall effect on the physical activity drops significantly. Furthermore, competitions with an equal mix of both men and women are more effective in increasing the level of activities. We leverage these insights to develop a statistical model to predict whether or not a competition will be particularly engaging with significant accuracy. Our models can serve as a guideline to help design more engaging competitions that lead to most beneficial behavioral changes.

==> content.tex <==
% !TEX root = paper-competition.tex




\section{Introduction}
\input{010intro}

\section{Related Work}
\input{020related}

\section{Dataset Description}
\input{030dataset}

\section{Does Competition Increase Activity?}
\input{040change_activity}

\section{What does it take to win a Competition?}
\input{045win_competition}

\section{What makes an interesting competition?}
\input{050interesting_competition}

\section{Predicting the effect of challenges}
\input{060prediction}

\section{Conclusion}
\input{070conclusion}
